Verifying Strong Eventual Consistency in $\delta$-CRDTs

Conflict-free replicated data types (CRDTs) are a natural structure with which to communicate information about a shared computation in a distributed setting where coordination overhead may not be tolerated, and individual participants are allowed to temporarily diverge from the overall computation. Within this setting, there are two classical approaches: state- and operation-based CRDTs. The former define a commutative, associative, and idempotent join operation, and their states a monotone join semi-lattice. State-based CRDTs may be further distinguished into classical- and $\delta$-state CRDTs. The former communicate their full state after each update, whereas the latter communicate only the changed state. Op-based CRDTs communicate operations (not state), thus making their updates non-idempotent. Whereas op-based CRDTs require little information to be exchanged, they demand relatively strong network guarantees (exactly-once message delivery), and state-based CRDTs suffer the opposite problem. Both satisfy strong eventual consistency (SEC). We posit that $\delta$-state CRDTs both (1) require less communication overhead from payload size, and (2) tolerate relatively weak network environments, making them an ideal candidate for real-world use of CRDTs. Our central intuition is a pair of reductions between state-, $\delta$-state, and op-based CRDTs. We formalize this intuition in the Isabelle interactive theorem prover and show that state-based CRDTs achieve SEC. We present a relaxed network model in Isabelle and show that state-based CRDTs still maintain SEC. Finally, we extend our work to show that $\delta$-state CRDTs maintain SEC when only communicating $\delta$-state fragments, even under relatively weak network conditions.

==> figures/theories/gcounter-comm-assoc.tex <==
\begin{isabellebody}
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gcounter{\isacharparenright}\ option{\isacharunderscore}max{\isacharunderscore}assoc{\isacharcolon}\isanewline
\ \ {\isachardoublequoteopen}option{\isacharunderscore}max\ a\ {\isacharparenleft}option{\isacharunderscore}max\ b\ c{\isacharparenright}\ {\isacharequal}\ option{\isacharunderscore}max\ {\isacharparenleft}option{\isacharunderscore}max\ a\ b{\isacharparenright}\ c{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}induction\ a{\isacharsemicolon}\ induction\ b{\isacharsemicolon}\ induction\ c{\isacharparenright}\isanewline
\ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto{\isacharparenright}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gcounter{\isacharparenright}\ option{\isacharunderscore}max{\isacharunderscore}commut{\isacharcolon}\ {\isachardoublequoteopen}option{\isacharunderscore}max\ a\ b\ {\isacharequal}\ option{\isacharunderscore}max\ b\ a{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}induction\ a{\isacharsemicolon}\ induction\ b{\isacharparenright}\isanewline
\ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto{\isacharparenright}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
\end{isabellebody}


==> figures/theories/gcounter.tex <==
\begin{isabellebody}%
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}id{\isacharparenright}\ state\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}id\ {\isasymRightarrow}\ int\ option{\isachardoublequoteclose}\isanewline
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}id{\isacharparenright}\ operation\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}id\ state{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ option{\isacharunderscore}max\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}int\ option\ {\isasymRightarrow}\ int\ option\ {\isasymRightarrow}\ int\ option{\isachardoublequoteclose}\ \ \isakeyword{where}\isanewline
{\isachardoublequoteopen}option{\isacharunderscore}max\ {\isacharparenleft}Some\ a{\isacharparenright}\ {\isacharparenleft}Some\ b{\isacharparenright}\ {\isacharequal}\ Some\ {\isacharparenleft}max\ a\ b{\isacharparenright}{\isachardoublequoteclose}\ {\isacharbar}\isanewline
{\isachardoublequoteopen}option{\isacharunderscore}max\ x\ None\ {\isacharequal}\ x{\isachardoublequoteclose}\ {\isacharbar}\isanewline
{\isachardoublequoteopen}option{\isacharunderscore}max\ None\ y\ {\isacharequal}\ y{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ update\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharprime}id\ state\ {\isasymRightarrow}\ {\isacharprime}id\ {\isasymRightarrow}\ {\isacharparenleft}int\ {\isasymRightarrow}\ int{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ operation{\isacharparenright}{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}update\ x\ i\ fn\ {\isacharequal}\ {\isacharparenleft}case\ {\isacharparenleft}x\ i{\isacharparenright}\ of\isanewline
\ \ \ \ \ \ None\ \ \ \ \ \ \ {\isasymRightarrow}\ x{\isacharparenleft}i\ {\isacharcolon}{\isacharequal}\ Some{\isacharparenleft}fn\ {\isadigit{0}}{\isacharparenright}{\isacharparenright}\isanewline
\ \ \ \ {\isacharbar}\ Some\ {\isacharparenleft}x{\isacharunderscore}i{\isacharparenright}\ {\isasymRightarrow}\ x{\isacharparenleft}i\ {\isacharcolon}{\isacharequal}\ Some{\isacharparenleft}fn\ x{\isacharunderscore}i{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ inc\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharprime}id\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ state{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ operation{\isacharparenright}{\isachardoublequoteclose}\ \ \isakeyword{where}\isanewline
{\isachardoublequoteopen}inc\ who\ st\ {\isacharequal}\ update\ st\ who\ {\isacharparenleft}{\isasymlambda}x{\isachardot}\ x\ {\isacharplus}\ {\isadigit{1}}{\isacharparenright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ dec\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharprime}id\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ state{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ operation{\isacharparenright}{\isachardoublequoteclose}\ \ \isakeyword{where}\isanewline
{\isachardoublequoteopen}dec\ who\ st\ {\isacharequal}\ update\ st\ who\ {\isacharparenleft}{\isasymlambda}x{\isachardot}\ x\ {\isacharminus}\ {\isadigit{1}}{\isacharparenright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ gcounter{\isacharunderscore}op\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharparenleft}{\isacharprime}id\ operation{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}id\ state{\isacharparenright}\ {\isasymrightharpoonup}\ {\isacharparenleft}{\isacharprime}id\ state{\isacharparenright}{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
{\isachardoublequoteopen}gcounter{\isacharunderscore}op\ theirs\ ours\ {\isacharequal}\ Some\ {\isacharparenleft}{\isasymlambda}\ x{\isachardot}\ option{\isacharunderscore}max\ {\isacharparenleft}theirs\ x{\isacharparenright}\ {\isacharparenleft}ours\ x{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{locale}\isamarkupfalse%
\ gcounter\ {\isacharequal}\ network{\isacharunderscore}with{\isacharunderscore}ops\ {\isacharunderscore}\ gcounter{\isacharunderscore}op\ {\isachardoublequoteopen}{\isasymlambda}\ x{\isachardot}\ None{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gcounter{\isacharparenright}\ option{\isacharunderscore}max{\isacharunderscore}assoc{\isacharcolon}\isanewline
\ \ {\isachardoublequoteopen}option{\isacharunderscore}max\ a\ {\isacharparenleft}option{\isacharunderscore}max\ b\ c{\isacharparenright}\ {\isacharequal}\ option{\isacharunderscore}max\ {\isacharparenleft}option{\isacharunderscore}max\ a\ b{\isacharparenright}\ c{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}induction\ a{\isacharsemicolon}\ induction\ b{\isacharsemicolon}\ induction\ c{\isacharparenright}\isanewline
\ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto{\isacharparenright}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gcounter{\isacharparenright}\ option{\isacharunderscore}max{\isacharunderscore}commut{\isacharcolon}\ {\isachardoublequoteopen}option{\isacharunderscore}max\ a\ b\ {\isacharequal}\ option{\isacharunderscore}max\ b\ a{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}induction\ a{\isacharsemicolon}\ induction\ b{\isacharparenright}\isanewline
\ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto{\isacharparenright}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
\isanewline
%
\endisadelimproof
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gcounter{\isacharparenright}\ {\isacharbrackleft}simp{\isacharbrackright}\ {\isacharcolon}\ {\isachardoublequoteopen}gcounter{\isacharunderscore}op\ x\ {\isasymrhd}\ gcounter{\isacharunderscore}op\ y\ {\isacharequal}\ gcounter{\isacharunderscore}op\ y\ {\isasymrhd}\ gcounter{\isacharunderscore}op\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto\ simp\ add{\isacharcolon}\ kleisli{\isacharunderscore}def\ option{\isacharunderscore}max{\isacharunderscore}assoc{\isacharparenright}\isanewline
\ \ \isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}simp\ add{\isacharcolon}\ option{\isacharunderscore}max{\isacharunderscore}commut{\isacharparenright}\isanewline
\ \ \isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
\end{isabellebody}


==> figures/theories/gset.tex <==
\begin{isabellebody}%
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}a{\isacharparenright}\ state\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}a\ set{\isachardoublequoteclose}\isanewline
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}a{\isacharparenright}\ operation\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}a\ state{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ insert\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharprime}a\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}a\ state{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}a\ operation{\isacharparenright}{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
{\isachardoublequoteopen}insert\ a\ as\ {\isacharequal}\ {\isacharbraceleft}\ a\ {\isacharbraceright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{fun}\isamarkupfalse%
\ gset{\isacharunderscore}op\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharparenleft}{\isacharprime}a\ operation{\isacharparenright}\ {\isasymRightarrow}\ {\isacharparenleft}{\isacharprime}a\ state{\isacharparenright}\ {\isasymrightharpoonup}\ {\isacharparenleft}{\isacharprime}a\ state{\isacharparenright}{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
{\isachardoublequoteopen}gset{\isacharunderscore}op\ a\ as\ {\isacharequal}\ Some\ {\isacharparenleft}\ as\ {\isasymunion}\ a\ {\isacharparenright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{locale}\isamarkupfalse%
\ gset\ {\isacharequal}\ network{\isacharunderscore}with{\isacharunderscore}ops\ {\isacharunderscore}\ gset{\isacharunderscore}op\ {\isachardoublequoteopen}{\isacharbraceleft}{\isacharbraceright}{\isachardoublequoteclose}\isanewline
\isanewline
\isacommand{lemma}\isamarkupfalse%
\ {\isacharparenleft}\isakeyword{in}\ gset{\isacharparenright}\ {\isacharbrackleft}simp{\isacharbrackright}\ {\isacharcolon}\ {\isachardoublequoteopen}gset{\isacharunderscore}op\ x\ {\isasymrhd}\ gset{\isacharunderscore}op\ y\ {\isacharequal}\ gset{\isacharunderscore}op\ y\ {\isasymrhd}\ gset{\isacharunderscore}op\ x{\isachardoublequoteclose}\isanewline
%
\isadelimproof
\ \ %
\endisadelimproof
%
\isatagproof
\isacommand{apply}\isamarkupfalse%
\ {\isacharparenleft}auto\ simp\ add{\isacharcolon}\ kleisli{\isacharunderscore}def{\isacharparenright}\isanewline
\isacommand{done}\isamarkupfalse%
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
\end{isabellebody}
\endinput

